Deep Architectures and Ensembles for Semantic Video Classification

This work addresses the problem of accurate semantic labelling of short videos. To this end, a multitude of different deep nets, ranging from traditional recurrent neural networks (LSTM, GRU), temporal agnostic networks (FV,VLAD,BoW), fully connected neural networks mid-stage AV fusion and others. Additionally, we also propose a residual architecture-based DNN for video classification, with state-of-the art classification performance at significantly reduced complexity. Furthermore, we propose four new approaches to diversity-driven multi-net ensembling, one based on fast correlation measure and three incorporating a DNN-based combiner. We show that significant performance gains can be achieved by ensembling diverse nets and we investigate factors contributing to high diversity. Based on the extensive YouTube8M dataset, we provide an in-depth evaluation and analysis of their behaviour. We show that the performance of the ensemble is state-of-the-art achieving the highest accuracy on the YouTube-8M Kaggle test data. The performance of the ensemble of classifiers was also evaluated on the HMDB51 and UCF101 datasets, and show that the resulting method achieves comparable accuracy with state-of-the-art methods using similar input features.

==> cover.tex <==
Our submission titled "Deep Architectures and Ensembles for Semantic Video Classification" concerns a detailed study of ensembling a wide range of Deep Neural Network architectures for semantic video classification.

This paper is based on our existing paper submitted to the CVPR2017 Workshop on Youtube-8M Large Scale Video Understanding, entitled: "Cultivating DNN Diversity for Large Scale Video Labelling". This has also been included with this manuscript. 

This submission significantly improves and extends from the above paper as follows:
1) Evaluation of a wide range of DNNs (including a novel architecture proposed here) for the purpose of video classification
2) Detailed analysis of the performance of the above DNNs, including diversity measures.
3) Evaluation of a number of different ensembling methods for optimally combining different DNNs.
The work in this paper produced an approach that significantly improves from the best entry for the Youtube-8M, with our approach scoring 85.12\% accuracy against the best entry of 84.9\%.
